A two-dimensional gallium phosphide optomechanical crystal in the resolved-sideband regime

Faithful quantum state transfer between telecom photons and microwave frequency mechanical oscillations necessitate a fast conversion rate and low thermal noise. Two-dimensional (2D) optomechanical crystals (OMCs) are favorable candidates that satisfy those requirements. 2D OMCs enable sufficiently high mechanical frequency (1$\sim$10 GHz) to make the resolved-sideband regime achievable, a prerequisite for many quantum protocols. It also supports higher thermal conductance than 1D structures, mitigating the parasitic laser absorption heating. Furthermore, gallium phosphide (GaP) is a promising material choice thanks to its large electronic bandgap of 2.26 eV, which suppresses two-photon absorption, and high refractive index $n$ = 3.05 at the telecom C-band, leading to a high-$Q$ optical mode. Here, we fabricate and characterize a 2D OMC made of GaP. We realize a high optical $Q$-factor of $7.9\times 10^{4}$, corresponding to a linewidth $\kappa/2\pi$ = 2.5 GHz at the telecom frequency 195.6 THz. This optical mode couples to several mechanical modes, whose frequencies all exceed the cavity linewidth. The most strongly coupled mode oscillates at 7.7 GHz, more than 3 times the optical linewidth, while achieving a substantial vacuum optomechanical coupling rate $g_{\mathrm{0}}/2\pi$ = 450 kHz. This makes the platform a promising candidate for a long-lived, deterministic quantum memory for telecom photons at low temperatures.

==> main_text.tex <==
\title{A two-dimensional gallium phosphide optomechanical crystal in the resolved-sideband regime}

\author{Sho Tamaki\authormark{1,2}, Mads Bjerregaard Kristensen\authormark{1,2}, Théo Martel\authormark{3}, Rémy Braive\authormark{3,4,5}, and Albert Schliesser\authormark{1,2,*}}

\address{\authormark{1}Niels Bohr Institute, University of Copenhagen, Blegdamsvej 17, Copenhagen 2100, Denmark\\
\authormark{2}Center for Hybrid Quantum Networks, Niels Bohr Institute, University of Copenhagen, Blegdamsvej 17, Copenhagen 2100, Denmark\\
\authormark{3}Centre de Nanosciences et de Nanotechnologies, CNRS, Université Paris Saclay, Palaiseau 91120, France\\
\authormark{4}Université Paris Cité, Paris 75006, France, France\\
\authormark{5}Institut Universitaire de France (IUF), Paris 75231, France}


\email{\authormark{*}albert.schliesser@nbi.ku.dk} %% email address is required; see note below about the corresponding author designation

% use {asbstract*} to suppress the copyright line. Copyright information will be added in production

\begin{abstract*} 
Faithful quantum state transfer between telecom photons and microwave frequency mechanical oscillations necessitate a fast conversion rate and low thermal noise.
Two-dimensional (2D) optomechanical crystals (OMCs) are favorable candidates that satisfy those requirements.
2D OMCs enable sufficiently high mechanical frequency (1$\sim$10 GHz) to make the resolved-sideband regime achievable, a prerequisite for many quantum protocols.
It also supports higher thermal conductance than 1D structures, mitigating the parasitic laser absorption heating.
Furthermore, gallium phosphide (GaP) is a promising material choice thanks to its large electronic bandgap of 2.26 eV, which suppresses two-photon absorption, and high refractive index $n$ = 3.05 at the telecom C-band, leading to a high-$Q$ optical mode.
Here, we fabricate and characterize a 2D OMC made of GaP.
We realize a high optical $Q$-factor of $7.9\times 10^{4}$, corresponding to a linewidth $\kappa/2\pi$ = 2.5 GHz at the telecom frequency 195.6 THz.
This optical mode couples to several mechanical modes, whose frequencies all exceed the cavity linewidth.
The most strongly coupled mode oscillates at 7.7 GHz, more than 3 times the optical linewidth, while achieving a substantial vacuum optomechanical coupling rate $g_{\mathrm{0}}/2\pi$ = 450 kHz.
This makes the platform a promising candidate for a long-lived, deterministic quantum memory for telecom photons at low temperatures.

\end{abstract*}

%%%%%%%%%%%%%%%%%%%%%%%%%%  body  %%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\begin{figure}[ht!]
\centering
\includegraphics[width=\linewidth]{Images/design.png}
\captionsetup{width=1\linewidth}
\caption{
Description of the OMC design. (a) Geometry of a unit cell. $( a,w,r,d )$ = (370, 120, 80, 577) nm and the thickness of 260 nm. The direction of the [100] crystalline axis is indicated by an arrow. (b) The 1st Brillouin zone. Band diagrams are simulated along the line surrounding the area indicated in yellow in the order of $\Gamma\rightarrow K \rightarrow M \rightarrow \Gamma$. 
(c) Mechanical band diagram. Relevant modes ($yz$-symmetric at the $\Gamma$ point) are highlighted by orange lines. The bandgap (4.77-7.94 GHz) is indicated in yellow.
(d) Optical band diagram. TE modes are highlighted by blue lines. The bandgap (181-238 THz) is indicated in yellow. The blue-shaded area shows the light cone. (e) SEM image of the full structure. The [100] crystalline axis lies parallel to the $x$-axis. The defect region is highlighted in blue. The horizontal gap, $\Delta_{\mathrm{gap}}$=600 nm, in the middle of the structure enables waveguide-like modes. (f) Schematic of the defect design. The $a$-parameter of snowflakes varies quadratically with a 3\% difference from the bulk value.}
\label{fig:design}
\end{figure}
Nanomechanical systems in the quantum regime have inspired researchers and engineers due to their potential applications ranging from ultra-sensitive force sensing to quantum communication\cite{gisler2024enhancingmembranebasedscanningforce,meesala_non-classical_2024}.
One specific application is an optomechanical quantum memory which uses a mechanical mode as a quantum coherent memory for telecom photons\cite{PhysRevLett.132.100802,Andreas2020,Fiaschi2021}, motivated by the long coherence time of micro-/nano-mechanical vibrations interacting effectively with telecom photons.
Quantum memory is a building block of the quantum repeater protocol\cite{Briegel-repeater-1998} that can surpass the current limit on transportation distance of optical quantum information through optical fibers ($\sim$600 km\cite{pittaluga_600-km_2021}).
The first quantum memory and repeater for light have been experimentally demonstrated with atomic gasses\cite{julsgaard_experimental_2004,yuan_experimental_2008}, and recently, optomechanical systems have achieved storage for telecomband wavelengths\cite{Andreas2020,Fiaschi2021}.
%Quantum memory is a building block of the quantum repeater protocol\cite{Briegel-repeater-1998} that can surpass the current limit on transportation distance of optical quantum information through optical fibers ($\sim$600 km\cite{pittaluga_600-km_2021}), and the first experimental demonstrations have been done with atomic gasses\cite{julsgaard_experimental_2004,yuan_experimental_2008}.
%Recently, this endeavor has been motivated by the long coherence time of micro-/nano-mechanical vibration interacting effectively with telecom photons in optomechanical systems.
%lthough quantum optomechanical memories have been achieved in silicon optomechanical crystals\cite{Andreas2020,Fiaschi2021}, deterministic write/readout of optical quantum states has yet to be demonstrated.
However, deterministic write/readout of optical states has yet to be demonstrated for practical quantum memories.

Deterministic storage requires a fast optomechanical conversion rate that matches the bandwidth of incoming photons ($\sim$200 MHz\cite{pedersen_near_2020}).
Generally speaking, the conversion rate scales with the number of intra-cavity photons and thus the intensity of the input laser\cite{aspelmeyer_cavity_2014}.
However, laser-absorption-induced heating at millikelvin temperature sets an upper limit for input laser power as it significantly degrades mechanical coherence.
This results in a trade-off between the conversion efficiency and the amount of thermal noise, thus restricting the performance of mechanical quantum memories and transducers\cite{Andreas2020,jiang_optically_2023,meesala_non-classical_2024}.
Accordingly, an optomechanical system robust against laser absorption heating is strongly desired.

Large efforts have been made in structural design to mitigate the problem.
It has been discovered that 2D structures can significantly reduce the laser-absorption-induced thermal bath occupancy compared to 1-dimensional structures\cite{HRen2020}.
Also, a sophisticated waveguide design that detaches the 2D mechanical mode from the local heat bath is capable of enhancing the performance of optomechanical transducers\cite{sonar_high-efficiency_2024}.
Another direction of effort is to seek a suitable material that inherently absorbs less laser light.
Recent studies \cite{Schneider2019, Stockill2019} have suggested gallium phosphide (GaP) as a favorable candidate due to (i) the large electronic bandgap of 2.26 eV exceeding the energy of two telecom photons ($\sim$1.6 eV), which can suppress the two-photon-absorption-induced thermalization, and (ii) the high refractive index $n=3.05$ enabling a high-$Q$ optical mode and large vacuum optomechanical coupling $g_{0}$.

Here, we design and characterize a 2D GaP optomechanical crystal (OMC).
\begin{comment}
The 2D structures can make thermal phonons dissipate faster, while its improved design allows large mechanical frequencies that can suppress thermal occupation.
\end{comment}
Our device hosts an optical resonance at 
$\omega_{\mathrm{o}}/2\pi$ = 195.55 THz, $\lambda_{\mathrm{o}}$ = 1533.1 nm with linewidth $\kappa/2\pi$ = 2.47 GHz which couples to 3 localized mechanical modes.
The most strongly coupled mechanical mode has a frequency $\Omega_{\mathrm{m}}/2\pi=$ 7.7 GHz and intrinsic linewidth $\Gamma_{\mathrm{m}}/2\pi$ = 4.9 MHz at room temperature, placing our device well in the resolved-sideband regime ($\Omega_{\mathrm{m}}>3\kappa$).
From a thermally calibrated measurement\cite{Gorodetsky2010} with different detunings, we infer a vacuum optomechanical coupling rate $g_0/2\pi$ = 452 kHz for this mode.



\section{Methods}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]
{Images/full_simulation.png}
\captionsetup{width=1\linewidth}
\caption{
Simulated $|g_{0}|$ for each mechanical eigenmode. Three dominant modes with high coupling rates are indicated by black lines at (5.75, 6.57, 7.85) GHz.
The inset (a) shows the absolute mechanical displacement of each mode.
(b) $E_{y}$ of the TE-like optical cavity mode with simulated frequency $\omega_{\mathrm{o}}/2\pi=192.7$ THz, which couples to those mechanical modes.
}
\label{fig:full-simu}
\end{figure}
Our OMC has snowflake-shaped holes\cite{Safavi-Naeini2014,PhysRevApplied.21.014015} in a periodic hexagonal lattice over the suspended GaP slab that opens bandgaps for both mechanical and optical modes. Fig$.$ \ref{fig:design}(a)
shows the dimension of a unit cell with parameters of $(a,w,r,d)$ = (370, 120, 80, 577) nm and a thickness of 260 nm.
This shape has more degrees of freedom for optical and mechanical mode engineering than the typical ellipses.
\begin{comment}
The optical mode mainly depends on the lattice constant $d$ and snowflake size $a$, while the mechanical mode is also sensitive to the width of a branch of the snowflake $w$. However, of course, each parameter more or less affects both modes at the same time.
\end{comment}
As for the mechanical properties, GaP has a Zincblende crystalline structure  $\bar{4}3m$, giving rise to anisotropy of mechanical properties with 4-fold rotational symmetry.
Therefore, the mechanical modes depend on the alignment of the OMC structure to the crystalline axis.
We align the snowflake so that one of the spikes points to the [100] crystalline axis to maximize the mechanical frequency while maintaining sufficient coupling strength.
We use elastic tensor components of $(C_{11},C_{12},C_{44})$ = (140.5, 62.0, 70.3) GPa for our simulation.

%The refractive index at telecom band $\lambda=$ 1550 nm is $n\sim$3.05, and we assume this value to be independent of wavelength in the simulation.
The band diagrams for both modes are simulated over $\Gamma\rightarrow K \rightarrow M \rightarrow \Gamma$ in the 1st Brillouin zone which is shown in Fig$.$ \ref{fig:design}(b,c).
As for the mechanical modes, we focus only on the modes with $yz$-symmetry at $\Gamma$ point, sharing parity with the optical mode.
Any mode without this symmetry results in small optomechanical coupling as the contribution from one side is canceled from the opposite side of the device.
%$x$-symmetry is unnecessary for the unit cell design as we introduce a line defect along the $x$-axis.
We find our design has a wide bandgap for relevant modes > 3 GHz around $\sim$6.5 GHz as well as a full bandgap > 1 GHz.
At the same time, the optical bands have a gap between around the telecom C-band (181-238 THz).

We then design the full device structure based on the unit cell simulations.
Subtracting a row of snowflakes, and adding a gap $\Delta_{\mathrm{gap}}$ = 600 nm shown in Fig$.$ \ref{fig:design}(e) creates waveguide modes with one-dimensional confinement.
The additional quadratic variation in snowflake size ($a$-parameter of the geometry) forms the defect region leading to two-dimensional confinement.
The gradual parameter variation gently shifts the bandgap from the mirror to the defect region resulting in high-$Q$ modes\cite{akahane_high-q_2003}.
Our device has a defect region formed over 8 snowflakes with the minimum $a$-parameter being only 3\% smaller than that of the mirror region as presented in Fig$.$ \ref{fig:design}(f).
\begin{comment}
It is connected to a single-mode waveguide (width=500 nm) which is further evanescently coupled to a tapered fiber for optical input/output. Our OMC supports the waveguide-like optical mode due to the gap $\Delta_{\mathrm{gap}}=$600 nm located at $y=0$, which confines the optical mode along the $x$-axis. The periodicity is broken by inducing the variation of the snowflake size as detailed in Fig$.$ \ref{fig:design}(f). We quadratically vary the $a$ parameter, which corresponds to the size of a snowflake spike, leading to the defect region. The smallest snowflakes are 3$\%$ smaller than those of the mirror region.
\end{comment}


We simulate optical and mechanical modes numerically with the finite element solver of COMSOL Multiphysics\cite{comsol} as shown in Fig$.$ \ref{fig:full-simu}.
The simulated TE-like optical mode Fig$.$ \ref{fig:full-simu}(b) has a telecom C-band frequency $\omega_{\mathrm{o}}/2\pi=192.7$ THz.
The vacuum optomechanical coupling rate $g_{0}$ is then computed by spatially integrating both modes considering the moving boundary (MB) and photoelastic (PE) contributions\cite{chan_optimized_2012,balram_moving_2014}.
MB contribution comes from the surface integral of the product of the electric field and the surface displacement, while PE is calculated by the volume integral of the product of the electric field and strain.
Simulated $g_{0}$'s are plotted in Fig$.$ \ref{fig:full-simu}(c) for each mechanical eigenmode.
There are 3 dominant mechanical modes at (5.75, 6.57, 7.85) GHz with sizable couplings $g_{0}/2\pi$ = (-718, -256, -983) kHz, with MB and PE contributions of $g_{\mathrm{mb}}/2\pi$ = (-305, -156, -755) kHz and $g_{\mathrm{pe}}/2\pi$ = (-414, -101, -228) kHz, respectively.
Note that the sign of the total coupling rate does not affect the characterization of the optomechanical device in this work.
We find both MB and PE contribute comparably to these modes thanks to the relatively high photoelastic constants of GaP $(p_{11}, p_{12}, p_{44})$ = (-0.23, -0.13, -0.10)\cite{mytsyk_elasto-optic_2015}, which are a factor of 2 larger than those of silicon\cite{biegelsen_photoelastic_1974}.
%Both mechanical and optical field profiles are shown in the insets.


\begin{comment}
Optomechanical confinement is achieved by carefully designing both mechanical and optical cavities by varying sizes of snowflakes $a$. As drawn in Fig$.$ \ref{fig:1}(d), the sizes change quadratically with a difference maximum of 3\% from \textit{mirror} to \textit{cavity} region. This variation achieves gradual mode matching between the cavity and mirror structures. This results in standing mechancial and optical modes (in Fig$.$ \ref{fig:1}(e)) with frequencies of $\Omega_{\mathrm{m}}/2\pi=$ 6.51 GHz and $\omega_{\mathrm{c}}/2\pi$ = 192 THz, respectively. Single-photon optomechanical coupling constant of $g_{0}/2\pi$ = 663 kHz is estimated by evaluating the moving boundary[] and photoelastic contributions[]. GaP has anisotropic photoelastic coefficients $(p_{11}, p_{12}, p_{44})$ = (-0.23, -0.13, -0.10). In order to make the most of the photoelasticity, our device is aligned so its waveguide is along with the [110] crystalline axis.

SEM images of our device are shown in Fig$.$ \ref{fig:2}(a). Fig$.$ \ref{fig:2}(b) shows the close-up image around our OMC structure. The white arrow in (b) is oriented to the [100] crystalline axis, and the OMC structure is rotated by 45$^\circ$ resulting in the waveguide being oriented to the [110] axis. Fig$.$ \ref{fig:2}(c,d) are schematic images of the tip and support of the waveguide respectively. The waveguide end is tapered to 120 nm width which creates the evanescent field of light which establishes optical coupling to an input fiber. The standard width of the waveguide is set to 500 nm which is narrow enough to be a single-mode waveguide. It is clamped in the middle with triangle supports to improve robustness. To reduce the effect of the clamp to waveguide mode, the width is enlarged to 900 nm around the clamps.
\end{comment}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Images/setup+fiber4.png}
\captionsetup{width=1\linewidth}
\caption{
Experimental setup. (a) SEM image of the OMC and waveguide for evanescent fiber coupling. The orange line indicates the fiber position. (b) Schematic of our measurement setup for device characterization. Orange and blue lines denote optical and electrical paths respectively. EOM: electro-optic phase modulator, EDFA: erbium-doped fiber amplifier, PD: photodetector, $\omega_{\mathrm{L}}$: laser frequency, and $\Omega_{\mathrm{c}}$: modulation frequency.
}
\label{fig:setup}
\end{figure}
The devices are fabricated on a 260-nm-thick GaP layer epitaxially grown on a gallium arsenide substrate (see supplemental for further details).
Fig$.$ \ref{fig:setup}(a) shows a scanning electron micrograph of the entire OMC and the access waveguide.
The 500 nm wide rectangular waveguide supports a single TE traveling mode with an effective index of 1.99.
We employ evanescent coupling between the waveguide and a tapered fiber\cite{tiecke_efficient_2015,burek_fiber-coupled_2017} for optical access (see supplemental for further details).
This configuration will allow us to make cryogenic packaging of the device\cite{zeng_cryogenic_2023} while suppressing the vibrational noise from the coupling fiber.
Our setup achieves a coupling efficiency as high as > 60\%.
Devices are characterized with the measurement setup shown in Fig$.$ \ref{fig:setup}(b).
The input light field comes from a tunable external cavity diode laser at frequency $\omega_{\mathrm{L}}$.
An electro-optic phase modulator (EOM) creates modulation sidebands at $\omega_{\mathrm{L}}\pm\Omega_{\mathrm{c}}$ used to determine the vacuum optomechanical coupling rate $g_{0}$.
A portion of the reflected light is sent to a photodetector (PD) to measure the optical spectrum and lock the laser detuning $\Delta$.
The other part of the reflected light is amplified by an erbium-doped fiber amplifier (EDFA) and then detected by a fast PD whose microwave signal is sent to a spectrum analyzer to characterize mechanical spectral properties.
All characterization is carried out at room temperature and ambient pressure.


\section{Results}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Images/spectra.png}
\captionsetup{width=1\linewidth}
\caption{
Characterization results. (a) Optical spectrum around resonance frequency $\omega_{\mathrm{o}}/2\pi$ = 195.55 THz, wavelength $\lambda_{\mathrm{o}}$ = 1533.1 nm showing a loaded quality factor $Q_{\mathrm{o}}$ = $7.92\times10^4$ ($\kappa/2\pi$ = 2.47 GHz). (b) Mechanical power spectral density (PSD) demonstrating 3 dominant modes around frequencies expected from the simulation. (c,d) Measured mechanical frequency and linewidth shift over detunings showing the dynamical backaction effect for modes 1 and 3. Estimated intrinsic frequency and linewidth are ($\Omega_{\mathrm{m}}/2\pi$, $\Gamma_{\mathrm{m}}/2\pi$) = (5.71 GHz, 4.57 MHz) for mode 1 and (7.65 GHz, 4.91 MHz) for mode 3. (e,f) Vacuum optomechanical coupling rate for each mode, yielding $g_{0}/2\pi$ = 231 (452) kHz for mode 1 (3), respectively.
}
\label{fig:result1}
\end{figure}
The optical spectrum is measured by scanning the laser frequency while acquiring the reflected optical power with a PD.
The laser power is set to a sufficiently small level to suppress the thermo-optical nonlinearity\cite{carmon_dynamical_2004}, which shifts the optical resonance towards a lower frequency depending on the power of a laser.
Fig$.$ \ref{fig:result1}(a) shows the measured optical reflection and the fitting curve
\begin{align}\label{eq:fitfunc}
    R(\Delta) = h - A\frac{(1-q^2)\kappa/2-q\Delta}{\kappa^2/4+\Delta^2},
\end{align}
derived from a model accounting for spurious back-reflection from the waveguide, detailed in the supplemental material.
Here, we define the offset $h$, amplitude parameter $A$, and the Fano parameter $q$, in addition to linewidth $\kappa$ and detuning $\Delta$.
%The optical spectrum shows Fano resonance because of parasitic back-reflection from the waveguide.
For optical resonance at $\lambda_{\mathrm{o}}$ = 1533.1 nm,  $\omega_{\mathrm{o}}/2\pi$ = 195.55 THz, this gives the loaded quality factor $Q_{\mathrm{o}}$ = $7.92\times10^4$ (linewidth $\kappa/2\pi$ = 2.47 GHz).
The output field is intensity-modulated at the mechanical frequency $\Omega_{\mathrm{m}}$ due to the combination of phase modulation by mechanical displacement and quadrature rotation by the optical cavity.
Fig$.$ \ref{fig:result1}(b) plots the power spectral density obtained by the spectrum analyzer.
We find 3 mechanical peaks at around $\Omega_{\mathrm{m}}/2\pi$ = 5.7, 6.5, 7.7 GHz, as predicted from the simulation.

To determine the precise values of the mechanical parameters, we analyze the dynamical backaction effects\cite{aspelmeyer_cavity_2014} on modes 1 and 3 by changing laser detuning $\Delta$ at fixed input power.
Measured shifts on mechanical frequencies and linewidths are plotted and fitted in Fig$.$ \ref{fig:result1}(c,d). The fitting curves are
\begin{align}
    \Omega_{\mathrm{eff}} &= \Omega_{\mathrm{m}} + \delta \Omega_{\mathrm{m}},\\
    \delta \Omega_{\mathrm{m}} &= g_{0}^{2}\frac{\kappa_{\mathrm{ex}}}{\Delta^{2}+(\kappa / 2)^{2}} \frac{P}{\hbar \omega_{\mathrm{L}}} \left(\frac{\Delta-\Omega_{\mathrm{m}}}{\kappa^{2} / 4+\left(\Delta-\Omega_{\mathrm{m}}\right)^{2}}+\frac{\Delta+\Omega_{\mathrm{m}}}{\kappa^{2} / 4+\left(\Delta+\Omega_{\mathrm{m}}\right)^{2}}\right),\\
    \Gamma_{\mathrm{eff}} &= \Gamma_{\mathrm{m}} + \delta \Gamma_{\mathrm{m}},\\
    \delta \Gamma_{\mathrm{m}}&=  g_{0}^{2}\frac{\kappa_{\mathrm{ex}}}{\Delta^{2}+(\kappa / 2)^{2}} \frac{P}{\hbar \omega_{\mathrm{L}}}\left(\frac{\kappa}{\kappa^{2} / 4+\left(\Delta+\Omega_{m}\right)^{2}}-\frac{\kappa}{\kappa^{2} / 4+\left(\Delta-\Omega_{m}\right)^{2}}\right),
\end{align}
\begin{comment}
\begin{align}
    \Omega_{\mathrm{eff}} &= \Omega_{\mathrm{m}} + \delta \Omega_{\mathrm{m}},\\
    \delta \Omega_{\mathrm{m}} &= g_{0}^{2}\frac{P}{\Delta^{2}+(\kappa / 2)^{2}}  \left(\frac{\Delta-\Omega_{\mathrm{m}}}{\kappa^{2} / 4+\left(\Delta-\Omega_{\mathrm{m}}\right)^{2}}+\frac{\Delta+\Omega_{\mathrm{m}}}{\kappa^{2} / 4+\left(\Delta+\Omega_{\mathrm{m}}\right)^{2}}\right),\\
    \Gamma_{\mathrm{eff}} &= \Gamma_{\mathrm{m}} + \delta \Gamma_{\mathrm{m}},\\
    \delta \Gamma_{\mathrm{m}}&=  g_{0}^{2}\frac{P}{\Delta^{2}+(\kappa / 2)^{2}} \left(\frac{\kappa}{\kappa^{2} / 4+\left(\Delta+\Omega_{\mathrm{m}}\right)^{2}}-\frac{\kappa}{\kappa^{2} / 4+\left(\Delta-\Omega_{\mathrm{m}}\right)^{2}}\right),
\end{align}
\end{comment}
where we define intrinsic frequency $\Omega_{\mathrm{m}}$, linewidth $\Gamma_{\mathrm{m}}$, input power to the optical cavity $P$, and external cavity loss $\kappa_{\mathrm{ex}}$.
We extract ($\Omega_{\mathrm{m}}/2\pi,\Gamma_{\mathrm{m}}/2\pi$) = ( 5.71 GHz, 4.57 MHz) for mode 1 and (7.65 GHz, 4.91 MHz) for mode 3.
Both modes are sideband-resolved ($\kappa < \Omega_{\mathrm{m}}$) which is a prerequisite for an effective optomechanical memory.
Note that the linewidth shifts for both modes are somewhat unclear because they are well sideband-resolved and the shifts are quite small in the region of $|\Delta|<\Omega_{\mathrm{m}}$.
%This does not negatively affect our characterization of mechanical parameters.

The optomechanical coupling rate $g_{0}$ is estimated by comparing the area below the mechanical noise power spectral density and the delta-function-like calibration tone generated by the EOM, whereby $g_{0}$ is calculated as\cite{Gorodetsky2010}:
\begin{align}
    g_{0} \approx \sqrt{ \frac{\phi_{0}^{2} \Omega_{\mathrm{c}}^{2}}{4\left\langle n_{\mathrm{th}}\right\rangle} \frac{S_{I I}^{\mathrm{meas}}\left(\Omega_{\mathrm{m}}\right) \Gamma_{\mathrm{m}} / 4}{S_{I I}^{\mathrm{meas}}\left(\Omega_{\mathrm{c}}\right) f_\mathrm{ENBW}}},
\end{align}
where $\phi_0$ is the phase modulation depth, $f_{\mathrm{ENBW}}$ the effective noise bandwidth of the spectrum analyzer in linear frequency, $S_{II}^{\mathrm{meas}}(\Omega)$ the symmetrized noise power spectral density at $\Omega$, and thermal mechanical occupation $\left\langle n_{\mathrm{th}}\right\rangle \approx k_{\mathrm{B}}T/ \hbar \Omega_{\mathrm{m}}$.
The modulation frequency $\Omega_{\mathrm{c}}/2\pi$ is set to no further from $\Omega_{\mathrm{m}}/2\pi$ than 40 MHz.
We measure $g_0$ in different laser detunings plotted in Fig$.$ \ref{fig:result1}(e,f) and obtain $g_0 /2\pi$ = 231±13 (452±32) kHz for mode 1 (3).


% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.6\linewidth]{Images/OMIT+OMIA.png}
% \caption{OMIT\& OMIA}
% \label{fig:OMIT}
% \end{figure}
%  Then we measure reflection with fine scanning around optical resonance by the VNA at a relatively strong input power. This shows the optomechanically induced transparency (OMIT) or amplification (OMIA) in red or blue detuning $\Delta\sim\pm\Omega_{\mathrm{m}}$ respectively. The broadened and compressed mechanical linewidths are due to the dynamical backaction, where the total linewidth is $\Gamma_{\mathrm{tot}}=\Gamma_{\mathrm{m}}\pm \Gamma_{\mathrm{opt}}$ for OMIT and OMIA respectively, and $\Gamma_{\mathrm{opt}}\equiv4g_{0}^2 \sqrt{\bar{n}_{\mathrm{c}}}/\kappa$. The broadened mechanical linewidth from OMIT gives us the optomechanical damping rate $\Gamma_{\mathrm{opt}}=2\pi\times1.0$ MHz, and the light-enhanced optomechanical coupling $g\equiv g_{0}\sqrt{\bar{n}_{\mathrm{c}}}=2\pi\times24.3$ MHz, where $\bar{n}_{\mathrm{c}}$ is the average number of the intra-cavity photon.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{comment}
\begin{table}[ht!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{|l|cc|cccc|c|}
\hline
\rowcolor[HTML]{b3cde0}
Mode& \multicolumn{1}{l}{Simulated}&  &\multicolumn{1}{l}{Measured}  & & & & \\ \hline
&$\Omega_{\mathrm{m}}/2\pi$ [GHz] & $(g_{\mathrm{mb}}+g_{\mathrm{pe}})/2\pi$ [kHz]&   $\Omega_{\mathrm{m}}/2\pi$ [GHz]& $\Gamma_{\mathrm{m}}/2\pi$ [MHz]& $\Omega_{\mathrm{m}}/\kappa$ & $g_{0}/2\pi$ [kHz] & $g_{0}^{\mathrm{Sim}}/g_{0}^{\mathrm{Meas}}$ \\ \hline
\multicolumn{1}{|l|}{This work}& & & & & & & \\
\multicolumn{1}{|c|}{Mode 1}& 5.75 & -305 - 414 &  5.71 $\pm$ 0.01 & 4.57 $\pm$ 0.04 & \textbf{2.31} & 231 $\pm$ 13&  3.1 \\
\multicolumn{1}{|c|}{Mode 2}& 6.57 & -156 - 101 &  6.50 $\pm$ 0.01 & 3.93 $\pm$ 0.41 & \textbf{2.63} & &\\
\multicolumn{1}{|c|}{Mode 3}& 7.85 & -755 - 228 &  7.65 $\pm$ 0.01 & 4.91 $\pm$ 0.03 & \textbf{3.10} & 452 $\pm$ 32 & 2.2 \\ \hline
\multicolumn{1}{|l|}{Schneider {\it{et al.}}\cite{Schneider2019}}& 2.84 & 35 + 725 &  2.90 & 3.13 & 1.61 & 370-680 & 2.1-1.1 \\ \hline
\multicolumn{1}{|l|}{Hönl {\it{et al.}}\cite{honl_microwave--optical_2022}}& & & & & & $(g_{0}^{\mathrm{blue}},g_{0}^{\mathrm{red}})/2\pi$ & \\
\multicolumn{1}{|c|}{Mode A}& 3.17 & 173 &  3.28 & 2.55 & 1.12 & (193, 189) & 0.9 \\
\multicolumn{1}{|c|}{Mode B}& 3.23 & 381 &  3.31 & 2.81 & 1.13 & (285, 281) & 1.3 \\
\multicolumn{1}{|c|}{Mode C}& 3.25 & 506 &  3.33 & 2.56 & 1.14 & (294, 291) & 1.7 \\ \hline
\multicolumn{1}{|l|}{Stockill {\it{et al.}}\cite{Stockill2019}}& 2.85 & 525 &  2.91 & \textbf{0.014} (@ 7 mK) & 0.56 & \textbf{845} & 0.6 \\ \hline
\end{tabular}}
\captionsetup{width=1\linewidth}
\caption{Comparison of simulated and measured parameters from different GaP OMCs.}
\label{table:result}
\end{table}
\end{comment}
\begin{table}[t]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{|l|cc|ccccc|}
\hline
\rowcolor[HTML]{b3cde0}
Mode& \multicolumn{1}{l}{Simulated}&  &\multicolumn{1}{l}{Measured}  & & & & \\ \hline
&$\Omega_{\mathrm{m}}/2\pi$ [GHz] & $|g_0|/2\pi$ [kHz]&   $\Omega_{\mathrm{m}}/2\pi$ [GHz]& $\Gamma_{\mathrm{m}}/2\pi$ [MHz]& $\Omega_{\mathrm{m}}/\kappa$ & $g_{0}/2\pi$ [kHz] & $C_\mathrm{0}=4g_{0}^2/\Gamma_{\mathrm{m}}\kappa$ \\ \hline
\multicolumn{1}{|l|}{This work}& & & & & & & \\
\multicolumn{1}{|c|}{Mode 1}& 5.75 & 719 &  5.71 $\pm$ 0.01 & 4.57 $\pm$ 0.04 & \textbf{2.31} & 231 $\pm$ 13&  $1.89\times10^{-5}$ \\
\multicolumn{1}{|c|}{Mode 2}& 6.57 & 257 &  6.50 $\pm$ 0.01 & 3.93 $\pm$ 0.41 & \textbf{2.63} & &\\
\multicolumn{1}{|c|}{Mode 3}& 7.85 & 983 &  7.65 $\pm$ 0.01 & 4.91 $\pm$ 0.03 & \textbf{3.10} & 452 $\pm$ 32 & $6.74\times10^{-5}$ \\ \hline
\multicolumn{1}{|l|}{Schneider {\it{et al.}}\cite{Schneider2019}}& 2.84 & 760 &  2.90 & 3.13 & 0.92 & 370-680 & $5.55$-$18.8\times10^{-5}$ \\ \hline
\multicolumn{1}{|l|}{Hönl {\it{et al.}}\cite{honl_microwave--optical_2022}}& & & & & &  & \\
\multicolumn{1}{|c|}{Mode A}& 3.17 & 173 &  3.28 & 2.55 & 1.12 & 191 & $1.96\times10^{-5}$ \\
\multicolumn{1}{|c|}{Mode B}& 3.23 & 381 &  3.31 & 2.81 & 1.13 & 283 & $3.90\times10^{-5}$ \\
\multicolumn{1}{|c|}{Mode C}& 3.25 & 506 &  3.33 & 2.56 & 1.14 & 293 & $4.59\times10^{-5}$ \\ \hline
\multicolumn{1}{|l|}{Stockill {\it{et al.}}\cite{Stockill2019}}& 2.85 & 525 &  2.91 & \textbf{0.014} (@ 7 mK) & 0.56 & \textbf{845} & $\boldsymbol{4.03\times10^{-2}}$ \\ \hline
\end{tabular}}
\captionsetup{width=1\linewidth}
\caption{Comparison of simulated and measured parameters from different GaP OMCs.}
\label{table:result}
\end{table}

Table \ref{table:result} compares parameters among GaP OMCs including this work and previously realized 1D devices.
Our mechanical modes show good agreement with simulations in their mechanical frequencies and they are 2 to 3 times higher than those of 1D OMCs of previous studies, thus realizing by far the largest $\Omega_{\mathrm{m}}/\kappa$ ratio of 3.10 for the mode 3.
The measured $g_0$'s are also comparably high.
We find that the measured $g_0$ for each mode is smaller than the simulated by a factor of $\sim$2-3.
Previous studies\cite{Schneider2019,honl_microwave--optical_2022} have also reported a factor of $\sim$2 difference.
We attribute this to our imperfect knowledge of the photoelastic constants of GaP in the telecom band. 
Additionally, the 2D structures' sensitivity to fabrication imperfection compared to 1D structures is still debatable (see supplemental for further details).
For the measured $g_{0}$ by Hönl {\it{et al.}}\cite{honl_microwave--optical_2022}, we take the mean value of blue- and red-detuned measurements.
We further compare the single-photon cooperativity $C_{\mathrm{0}}=4g_{0}^2/\Gamma_{\mathrm{m}}\kappa$, which corresponds to an optomechanical cooperativity per cavity photon.
Our device achieves $C_{\mathrm{0}}=6.74\times10^{-5}$ for mode 3 which is one of the highest among the room temperature GaP OMCs studied so far.
This is quite an encouraging result considering applications such as quantum memory.
As previously demonstrated in a silicon OMC\cite{HRen2020,sonar_high-efficiency_2024}, 2D structures have an advantage on thermalization at a given laser power.
Therefore, we may deduce that our device can achieve higher quantum cooperativity $C_{\mathrm{q}}=n_{\mathrm{cav}}C_{\mathrm{0}}/n_{\mathrm{th}}$ than 1D GaP OMC at cryogenic temperature as we can input stronger power, thus more cavity photons $n_{\mathrm{cav}}$.
%Here we define the simulated (measured) coupling rate $g_{0}^{\mathrm{Sim (Meas)}}$ and measured value on blue (red) detuning $g_{0}^{\mathrm{blue (red)}}$.



\begin{comment}
\section{Discussion}
Previous studies on silicon OMCs\cite{HRen2020} have revealed the superior performance of 2D structures over 1Ds in terms of thermalization.
An absorption-induced thermal bath occupancy $n_{\mathrm{p}}=1.1\times n_{\mathrm{cav}}^{0.3}$ has been reported at cryogenic temperature ($\sim$10 mK) on a 2D device with the number of cavity photons of $n_{\mathrm{cav}}<10^4$.
This result is 7 times smaller than that of 1D OMC thanks to the enhanced thermal conductance.
Another study on GaP OMC\cite{Schneider2019} at room temperature has shown at least 5 times smaller optical absorption rate than silicon in the same photon number range.
Combining those naively suggests that our device will be allowed to host 5 times more cavity photons than 2D Silicon OMCs while suppressing the thermalization.
As the photon-phonon transition rate scales with $g_{0}\sqrt{n_{\mathrm{cav}}}$, more photons are beneficial to increase the rate and to reduce the bandwidth mismatch from single-photons.
However, it should be noted that heating dynamics at cryogenic temperature is still not yet fully understood. The temperature rise at room temperature is linear to the input power which is different from that is reported in cryogenic experiments.
\end{comment}

\section{Conclusion}
We design and characterize a GaP optomechanical crystal with a 2D geometry.
The careful design realizes the highest $\Omega_{\mathrm{m}}/\kappa$ ratio > 3 yet achieved in GaP OMCs, which places well in the sideband-resolved regime.
This is one of the requirements for faithful photon-phonon conversion.
From dynamical backaction measurements, we precisely characterize the mechanical properties.
The most strongly coupled mode achieves a large vacuum optomechanical coupling rate $g_{0}/2\pi$=452 kHz to a telecom optical cavity mode.
The measured $g_{0}$'s are smaller compared to the simulation results by similar factors that have previously been reported in one-dimensional devices\cite{Schneider2019,honl_microwave--optical_2022}.
We speculate this is a common problem due to the imperfect knowledge of the photoelastic constant of GaP for telecom photons.
In addition, 2D designs may be more vulnerable to fabrication imperfections such as uneven sidewalls, because of the structural complexity.
%Rigorously speaking, we observe slightly larger reductions of $g_{0}$ by the largest factor of 3.1, which we attribute to the fact that 2D designs are more vulnerable to fabrication imperfection e.g., uneven sidewalls, because of the structural complexity.

We expect our device to be less susceptible to laser heating thanks to the 2D structural design and GaP material properties, compared to other OMC devices.
The design is expected to diffuse thermal phonons faster than 1D thus lowering absorption-induced thermal occupation as previously reported on silicon devices\cite{HRen2020}.
We further assume that the recently reported waveguide design\cite{sonar_high-efficiency_2024}, which successfully decouples the local waveguide heat bath from the OMC cavity, is capable of further enhancing the thermalization performance of our device.
Although GaP is a quite promising material considering its large electronic bandgap, additional thin Al$_2$O$_3$ layer deposition may result in better suppression of optical absorption at the surfaces as reported on GaAs OMCs\cite{forsch_microwave--optics_2020}.
On top of that, there is still room for improving the evanescent fiber-waveguide coupling efficiency, which is crucial for deterministic photon-phonon conversion, by optimizing the waveguide design and the fiber etching process.
A coupling efficiency of 97\% has been reported in a diamond nanobeam photonic crystal\cite{tiecke_efficient_2015}.
This coupling configuration will allow us to make a cryogenic packaging of the device for millikelvin temperature experiments\cite{zeng_cryogenic_2023}.
With those further improvements and the currently demonstrated optomechanical memory protocol\cite{PhysRevLett.132.100802}, our device opens the possibility for deterministic quantum memories for single telecom photons.

Previous studies on silicon OMCs\cite{HRen2020} have revealed the superior performance of 2D structures over 1Ds in terms of thermalization.
An absorption-induced thermal bath occupancy $n_{\mathrm{p}}=1.1\times n_{\mathrm{cav}}^{0.3}$ has been reported at cryogenic temperature ($\sim$10 mK) on a 2D device with the number of cavity photons of $n_{\mathrm{cav}}<10^4$.
This result is 7 times smaller than that of 1D OMC thanks to the enhanced thermal conductance.
Another study on GaP OMC\cite{Schneider2019} at room temperature has shown at least 5 times smaller optical absorption rate than silicon in the same photon number range.
Combining those naively suggests that our device will be allowed to host 5 times more cavity photons than 2D Silicon OMCs while suppressing the thermalization.
As the photon-phonon conversion rate scales with $g_{0}^{2}n_{\mathrm{cav}}/\kappa$, more photons are beneficial to increase the conversion rate and match the bandwidth of single-photons.
However, it should be noted that heating dynamics at cryogenic temperature is still not yet fully understood. The temperature rise at room temperature is linear to the input power\cite{Schneider2019} which is different from that is reported in cryogenic experiments\cite{HRen2020}.

\section*{Acknowledgements}
This work was supported by the European Research Council project PHOQS (Grant No. 101002179), the Novo Nordisk Foundation (Grant No. NNF20OC0061866), the Danish National Research Foundation (Center of Excellence “Hy-Q”), the Independent Research Fund Denmark (Grant No. 1026-00345B), the French RENATECH network, as well as the CNRS-KU grant (Grant No. C2N UMR9001).

%\section*{Acknowledgements}
%The authors acknowledge helpful discussions with Anders S. Sørensen regarding the theoretical modeling.

\section*{Supplemental document}
See Supplement 1 for supporting content.



%%%%%%%%%%%%%%%%%%%%%%% References %%%%%%%%%%%%%%%%%%%%%%%%%
%\end{comment}



